HELPER-X: A Unified Instructable Embodied Agent to Tackle Four Interactive Vision-Language Domains with Memory-Augmented Language Models

Recent research on instructable agents has used memory-augmented Large Language Models (LLMs) as task planners, a technique that retrieves language-program examples relevant to the input instruction and uses them as in-context examples in the LLM prompt to improve the performance of the LLM in inferring the correct action and task plans. In this technical report, we extend the capabilities of HELPER, by expanding its memory with a wider array of examples and prompts, and by integrating additional APIs for asking questions. This simple expansion of HELPER into a shared memory enables the agent to work across the domains of executing plans from dialogue, natural language instruction following, active question asking, and commonsense room reorganization. We evaluate the agent on four diverse interactive visual-language embodied agent benchmarks: ALFRED, TEACh, DialFRED, and the Tidy Task. HELPER-X achieves few-shot, state-of-the-art performance across these benchmarks using a single agent, without requiring in-domain training, and remains competitive with agents that have undergone in-domain training.

==> 8_prompts.tex <==
\lstset{escapeinside={<@}{@>}, language=}
\onecolumn\begin{lstlisting}[caption={Full list of user personalization requests for the user personalization evaluation.},captionpos=t,label={user_pers_app}] 
<@\textcolor{orange}{original input to LLM:}@>
[['Driver', 'What is my task?'], ['Commander', "Make me a sandwich. The name of this sandwich is called the Larry sandwich. The sandwich has two slices of toast, 3 slices of tomato, and 3 slice of lettuce on a clean plate."]]
[['Driver', 'What is my task?'], ['Commander', 'Make me a salad. The name of this salad is called the David salad. The salad has two slices of tomato and three slices of lettuce on a clean plate.']]
[['Driver', 'What is my task?'], ['Commander', "Make me a salad. The name of this salad is called the Dax salad. The salad has two slices of cooked potato. You'll need to cook the potato on the stove. The salad also has a slice of lettuce and a slice of tomato. Put all components on a clean plate."]]
[['Driver', 'What is my task?'], ['Commander', 'Make me breakfast. The name of this breakfast is called the Mary breakfast. The breakfast has a mug of coffee, and two slices of toast on a clean plate.']]
[['Driver', 'What is my task?'], ['Commander', 'Make me breakfast. The name of this breakfast is called the Lion breakfast. The breakfast has a mug of coffee, and four slices of tomato on a clean plate.']]
[['Driver', 'What is my task?'], ['Commander', 'Rearrange some objects. The name of this rearrangement is called the Lax rearrangement. Place three pillows on the sofa.']]
[['Driver', 'What is my task?'], ['Commander', 'Rearrange some objects. The name of this rearrangement is called the Pax rearrangement. Place two pencils and two pens on the desk.']]
[['Driver', 'What is my task?'], ['Commander', 'Clean some objects. The name of this cleaning is called the Gax cleaning. Clean two plates and two cups.']]
[['Driver', 'What is my task?'], ['Commander', "Make me a sandwich. The name of this sandwich is called the Gabe sandwich. The sandwich has two slices of toast, 2 slices of tomato, and 1 slice of lettuce on a clean plate."]]
[['Driver', 'What is my task?'], ['Commander', 'Clean some objects. The name of this cleaning is called the Kax cleaning. Clean a mug and a pan.']]

<@\textcolor{orange}{No change:}@>
"Make me the Larry sandwich"
"Make me the David salad"
"Make me the Dax salad"
"Make me the Mary breakfast"
"Make me the Lion breakfast"
"Complete the Lax rearrangement"
"Complete the Pax rearrangement"
"Perform the Gax cleaning"
"Make me the Gabe sandwich"
"Perform the Kax cleaning"

<@\textcolor{orange}{One change:}@>
"Make me the Larry sandwich with four slices of lettuce"
"Make me the David salad with a slice of potato"
"Make me the Dax salad without lettuce"
"Make me the Mary breakfast with no coffee"
"Make me the Lion breakfast with three slice of tomato"
"Complete the Lax rearrangement with two pillows"
"Complete the Pax rearrangement but use one pencil instead of the the two pencils"
"Perform the Gax cleaning with three plates instead of two"
"Make me the Gabe sandwich with only 1 slice of tomato"
"Perform the Kax cleaning with only a mug"

<@\textcolor{orange}{Two changes:}@>
"Make me the Larry sandwich with four slices of lettuce and two slices of tomato"
"Make me the David salad but add a slice of potato and add one slice of egg"
"Make me the Dax salad without lettuce and without potato"
"Make me the Mary breakfast with no coffee and add an egg"
"Make me the Lion breakfast with three slice of tomato and two mugs of coffee"
"Complete the Lax rearrangement with two pillows and add a remote"
"Complete the Pax rearrangement but use one pencil instead of the two pencils and add a book"
"Perform the Gax cleaning with three plates instead of the two plates and include a fork"
"Make me the Gabe sandwich with only 1 slice of tomato and two slices of lettuce"
"Perform the Kax cleaning without the pan and include a spoon"

<@\textcolor{orange}{Three changes:}@>
"Make me the Larry sandwich with four slices of lettuce, two slices of tomato, and place all components directly on the countertop"
"Make me the David salad and add a slice of potato, add one slice of egg, and bring a fork with it"
"Make me the Dax salad without lettuce, without potato, and add an extra slice of tomato"
"Make me the Mary breakfast with no coffee, add an egg, and add a cup filled with water"
"Make me the Lion breakfast with three slice of tomato, two mugs of coffee, and add a fork"
"Complete the Lax rearrangement with two pillows, a remote, and place it on the arm chair instead"
"Complete the Pax rearrangement but use one pencil instead of the two pencils and include a book and a baseball bat"
"Perform the Gax cleaning with three plates instead of the two plates, include a fork, and do not clean any cups"
"Make me the Gabe sandwich with only 1 slice of tomato, two slices of lettuce, and add a slice of egg"
"Perform the Kax cleaning without the pan, include a spoon, and include a pot"
\end{lstlisting}

\lstset{escapeinside=, language=Python}

% \paragraph{API} Full API for the parametrized macro-actions $G$ used in the prompts.
% \label{prompt1}
\onecolumn\begin{lstlisting}[caption={Full API for the parametrized macro-actions $G$ used in the prompts.},captionpos=t,label={prompt1}] 
class InteractionObject:
    """
    This class represents an expression that uniquely identifies an object in the house.
    """
    def __init__(self, object_class: str, landmark: str = None, attributes: list = []):
        '''
        object_class: object category of the interaction object (e.g., "Mug", "Apple")
        landmark: (optional if mentioned) landmark object category that the interaction object is in relation to (e.g., "CounterTop" for "apple is on the countertop")
        attributes: (optional) list of strings of desired attributes for the object. These are not necessarily attributes that currently exist, but ones that the object should eventually have. Attributes can only be from the following: "toasted", "clean", "cooked"
        '''
        self.object_class = object_class
        self.landmark = landmark
        self.attributes = attributes

    def pickup(self):
        """pickup the object.

        This function assumes the object is in view.

        Example:
        dialogue: <Commander> Go get the lettuce on the kitchen counter.
        Python script:
        target_lettuce = InteractionObject("Lettuce", landmark = "CounterTop")
        target_lettuce.go_to()
        target_lettuce.pickup()
        """
        pass

    def place(self, landmark_name):
        """put the interaction object on the landmark_name object.

        landmark_name must be a class InteractionObject instance

        This function assumes the robot has picked up an object and the landmark object is in view.

        Example:
        dialogue: <Commander> Put the lettuce on the kitchen counter.
        Python script:
        target_lettuce = InteractionObject("Lettuce", landmark = "CounterTop")
        target_lettuce.go_to()
        target_lettuce.pickup()
        target_countertop = InteractionObject("CounterTop")
        target_countertop.go_to()
        target_lettuce.place(target_countertop)
        """
        pass

    def slice(self):
        """slice the object into pieces.

        This function assumes the agent is holding a knife and the agent has navigated to the object using go_to().

        Example:
        dialogue: <Commander> Cut the apple on the kitchen counter.
        Python script:
        target_knife = InteractionObject("Knife") # first we need a knife to slice the apple with
        target_knife.go_to()
        target_knife.pickup()
        target_apple = InteractionObject("Apple", landmark = "CounterTop")
        target_apple.go_to()
        target_apple.slice()
        """
        pass

    def toggle_on(self):
        """toggles on the interaction object.

        This function assumes the interaction object is already off and the agent has navigated to the object.
        Only some landmark objects can be toggled on. Lamps, stoves, and microwaves are some examples of objects that can be toggled on.

        Example:
        dialogue: <Commander> Turn on the lamp.
        Python script:
        target_floorlamp = InteractionObject("FloorLamp")
        target_floorlamp.go_to()
        target_floorlamp.toggle_on()
        """
        pass

    def toggle_off(self):
        """toggles off the interaction object.

        This function assumes the interaction object is already on and the agent has navigated to the object.
        Only some objects can be toggled off. Lamps, stoves, and microwaves are some examples of objects that can be toggled off.

        Example:
        dialogue: <Commander> Turn off the lamp.
        Python script:
        target_floorlamp = InteractionObject("FloorLamp")
        target_floorlamp.go_to()
        target_floorlamp.toggle_off()
        """
        pass

    def go_to(self):
        """Navigate to the object

        """
        pass

    def open(self):
        """open the interaction object.

        This function assumes the landmark object is already closed and the agent has already navigated to the object.
        Only some objects can be opened. Fridges, cabinets, and drawers are some example of objects that can be closed.

        Example:
        dialogue: <Commander> Get the lettuce in the fridge.
        Python script:
        target_fridge = InteractionObject("Fridge")
        target_lettuce = InteractionObject("Lettuce", landmark = "Fridge")
        target_fridge.go_to()
        target_fridge.open()
        target_lettuce.pickup()
        """
        pass

    def close(self):
        """close the interaction object.

        This function assumes the object is already open and the agent has already navigated to the object.
        Only some objects can be closed. Fridges, cabinets, and drawers are some example of objects that can be closed.
        """
        pass
    
    def clean(self):
        """wash the interaction object to clean it in the sink.

        This function assumes the object is already picked up.

        Example:
        dialogue: <Commander> Clean the bowl
        Python script:
        target_bowl = InteractionObject("Bowl", attributes = ["clean"])
        target_bowl.clean()
        """
        pass

    def put_down(self):
        """puts the interaction object currently in the agent's hand on the nearest available receptacle

        This function assumes the object is already picked up.
        This function is most often used when the holding object is no longer needed, and the agent needs to pick up another object
        """
        pass

    def pour(self, landmark_name):
        """pours the contents of the interaction object into the landmark object specified by the landmark_name argument

        landmark_name must be a class InteractionObject instance

        This function assumes the object is already picked up and the object is filled with liquid. 
        """
        pass

    def fill_up(self):
        """fill up the interaction object with water

        This function assumes the object is already picked up. Note that only container objects can be filled with liquid. 
        """
        pass

    def pickup_and_place(self, landmark_name):
        """go_to() and pickup() this interaction object, then go_to() and place() the interaction object on the landmark_name object.

        landmark_name must be a class InteractionObject instance
        """
        pass

    def empty(self):
        """Empty the object of any other objects on/in it to clear it out. 

        Useful when the object is too full to place an object inside it.

        Example:
        dialogue: <Commander> Clear out the sink. 
        Python script:
        target_sink = InteractionObject("Sink")
        target_sink.empty()
        """
        pass

    def cook(self):
        """Cook the object

        Example:
        dialogue: <Commander> Cook the potato. 
        Python script:
        target_potato = InteractionObject("Potato", attributes = ["cooked"])
        target_potato.cook()
        """
        pass

    def toast(self):
        """Toast a bread slice in a toaster

        Toasting is only supported with slices of bread

        Example:
        dialogue: <Commander> Get me a toasted bread slice. 
        Python script:
        target_breadslice = InteractionObject("BreadSliced", attributes = ["toasted"])
        target_breadslice.toast()
        """
        pass
\end{lstlisting}

% \paragraph{Corrective API} Full Corrective API for the parametrized corrective macro-actions $G_{corrective}$ used in the prompts.
\onecolumn\begin{lstlisting}[caption={Full Corrective API for the parametrized corrective macro-actions $G_{corrective}$ used in the prompts.},captionpos=t,label={prompt2}]
class AgentCorrective:
    '''
    This class represents agent corrective actions that can be taken to fix a subgoal error
    Example usage:
    agent = AgentCorrective()
    agent.move_back()
    '''

    def move_back(self):
        """Step backwards away from the object

        Useful when the object is too close for the agent to interact with it
        """
        pass

    def move_closer(self):
        """Step forward to towards the object to get closer to it

        Useful when the object is too far for the agent to interact with it
        """
        pass

    def move_alternate_viewpoint(self):
        """Move to an alternate viewpoint to look at the object

        Useful when the object is occluded or an interaction is failing due to collision or occlusion.
        """
        pass
\end{lstlisting}

\lstset{language=}

% \paragraph{$\planner$ Prompt} Full Prompt for the $\planner$. \{\} indicates areas that are replaced in the prompt.
\onecolumn\begin{lstlisting}[caption={Full Prompt for the planner. \{\} indicates areas that are replaced in the prompt.},captionpos=t,label={prompt3}]
You are an adept at translating human dialogues into sequences of actions for household robots. Given a dialogue between a <Driver> and a <Commander>, you convert the conversation into a Python program to be executed by a robot.

{API}

Write a script using Python and the InteractionObject class and functions defined above that could be executed by a household robot. 

{RETRIEVED_EXAMPLES}

Adhere to these stringent guidelines:
1. Use only the classes and functions defined previously. Do not create functions that are not provided above.
2. Make sure that you output a consistent plan. For example, opening of the same object should not occur in successive steps.
3. Make sure the output is consistent with the proper affordances of objects. For example, a couch cannot be opened, so your output should never include the open() function for this object, but a fridge can be opened. 
4. The input is dialogue between <Driver> and <Commander>. Interpret the dialogue into robot actions. Do not output any dialogue.
5. Object categories should only be chosen from the following classes: ShowerDoor, Cabinet, CounterTop, Sink, Towel, HandTowel, TowelHolder, SoapBar, ToiletPaper, ToiletPaperHanger, HandTowelHolder, SoapBottle, GarbageCan, Candle, ScrubBrush, Plunger, SinkBasin, Cloth, SprayBottle, Toilet, Faucet, ShowerHead, Box, Bed, Book, DeskLamp, BasketBall, Pen, Pillow, Pencil, CellPhone, KeyChain, Painting, CreditCard, AlarmClock, CD, Laptop, Drawer, SideTable, Chair, Blinds, Desk, Curtains, Dresser, Watch, Television, WateringCan, Newspaper, FloorLamp, RemoteControl, HousePlant, Statue, Ottoman, ArmChair, Sofa, DogBed, BaseballBat, TennisRacket, VacuumCleaner, Mug, ShelvingUnit, Shelf, StoveBurner, Apple, Lettuce, Bottle, Egg, Microwave, CoffeeMachine, Fork, Fridge, WineBottle, Spatula, Bread, Tomato, Pan, Cup, Pot, SaltShaker, Potato, PepperShaker, ButterKnife, StoveKnob, Toaster, DishSponge, Spoon, Plate, Knife, DiningTable, Bowl, LaundryHamper, Vase, Stool, CoffeeTable, Poster, Bathtub, TissueBox, Footstool, BathtubBasin, ShowerCurtain, TVStand, Boots, RoomDecor, PaperTowelRoll, Ladle, Kettle, Safe, GarbageBag, TeddyBear, TableTopDecor, Dumbbell, Desktop, AluminumFoil, Window, LightSwitch, AppleSliced, BreadSliced, LettuceSliced, PotatoSliced, TomatoSliced
6. You can only pick up one object at a time. If the agent is holding an object, the agent should place or put down the object before attempting to pick up a second object.
7. Each object instance should instantiate a different InteractionObject class even if two object instances are the same object category. 
Follow the output format provided earlier. Think step by step to carry out the instruction.

Write a Python script that could be executed by a household robot for the following:
dialogue: {command}
Python script: 
\end{lstlisting}

% \paragraph{$\rectifier$ Prompt} Full Prompt for the $\rectifier$. \{\} indicates areas that are replaced in the prompt.
\onecolumn\begin{lstlisting}[caption={Full Prompt for the rectifier. \{\} indicates areas that are replaced in the prompt.},captionpos=t,label={prompt4}]
You are an excellent interpreter of human instructions for household tasks. Given a failed action subgoal by a household robot, dialogue instructions between robot <Driver> and user <Commander>, and information about the environment and failure, you provide a sequence of robotic subgoal actions to overcome the failure.

{API}

{API_CORRECTIVE}

Information about the failure and environment are given as follows:
Failed subgoal: The robotic subgoal for which the failure occured.
Execution error: feedback as to why the failed subgoal occurred.
Input dialogue: full dialogue instructions between robot <Driver> and user <Commander> for the complete task. This may or may not be useful.

I will give you examples of the input and output you will generate.
{retrieved_plans}

Fix the subgoal exectuion error using only the InteractionObject class and functions defined above that could be executed by a household robot. Follow these rules very strictly:
1. Important! Use only the classes and functions defined previously. Do not create functions or additional code that are not provided in the above API. Do not include if-else statements.
2. Important! Make sure that you output a consistent plan. For example, opening of the same object should not occur in successive steps.
3. Important! Make sure the output is consistent with the proper affordances of objects. For example, a couch cannot be opened, so your output should never include the open() function for this object, but a fridge can be opened. 
4. Important! The dialogue is between <Driver> and <Commander>. The dialogue may or may not be helpful. Do not output any dialogue.
5. Important! Object classes should only be chosen from the following classes: ShowerDoor, Cabinet, CounterTop, Sink, Towel, HandTowel, TowelHolder, SoapBar, ToiletPaper, ToiletPaperHanger, HandTowelHolder, SoapBottle, GarbageCan, Candle, ScrubBrush, Plunger, SinkBasin, Cloth, SprayBottle, Toilet, Faucet, ShowerHead, Box, Bed, Book, DeskLamp, BasketBall, Pen, Pillow, Pencil, CellPhone, KeyChain, Painting, CreditCard, AlarmClock, CD, Laptop, Drawer, SideTable, Chair, Blinds, Desk, Curtains, Dresser, Watch, Television, WateringCan, Newspaper, FloorLamp, RemoteControl, HousePlant, Statue, Ottoman, ArmChair, Sofa, DogBed, BaseballBat, TennisRacket, VacuumCleaner, Mug, ShelvingUnit, Shelf, StoveBurner, Apple, Lettuce, Bottle, Egg, Microwave, CoffeeMachine, Fork, Fridge, WineBottle, Spatula, Bread, Tomato, Pan, Cup, Pot, SaltShaker, Potato, PepperShaker, ButterKnife, StoveKnob, Toaster, DishSponge, Spoon, Plate, Knife, DiningTable, Bowl, LaundryHamper, Vase, Stool, CoffeeTable, Poster, Bathtub, TissueBox, Footstool, BathtubBasin, ShowerCurtain, TVStand, Boots, RoomDecor, PaperTowelRoll, Ladle, Kettle, Safe, GarbageBag, TeddyBear, TableTopDecor, Dumbbell, Desktop, AluminumFoil, Window, LightSwitch, AppleSliced, BreadSliced, LettuceSliced, PotatoSliced, TomatoSliced
6. Important! You can only pick up one object at a time. If the agent is holding an object, the agent should place or put down the object before attempting to pick up a second object.
7. Important! Each object instance should instantiate a different InteractionObject class even if two object instances are the same object category. 
8. Important! Your plan should ONLY fix the failed subgoal. Do not include plans for other parts of the dialogue or future plan that are irrelevant to the execution error and failed subgoal. 
9. Important! output "do_nothing()" if the agent should not take any corrective actions.
Adhere to the output format I defined above. Think step by step to carry out the instruction.

Make use of the following information to help you fix the failed subgoal:
Failed subgoal: ...
Execution error: ...
Input dialogue: ...

You should respond in the following format:
Explain: Are there any steps missing to complete the subgoal? Why did the failed subgoal occur? What does the execution error imply for how to fix your future plan?
Plan (Python script): A Python script to only fix the execution error.

Explain: 
\end{lstlisting}

% \paragraph{$\locator$ Prompt} Full Prompt for the $\locator$. \{\} indicates areas that are replaced in the prompt.
\onecolumn\begin{lstlisting}[caption={Full Prompt for the $\locator$. \{\} indicates areas that are replaced in the prompt.},captionpos=t,label={prompt5}]
You are a household robot trying to locate objects within a house.
You will be given a target object category, your task is to output the top 3 most likely object categories that the target object category is likely to be found near: {OBJECT_CLASSES}
For your answer, take into account commonsense co-occurances of objects within a house and (if relevant) any hints given by the instruction dialogue between the robot <Driver> and user <Commander>.

For example, if given the target object category is "Knife" and the following dialogue: "<Commander> hi, make a slice of tomato. <Driver> where is the tomato? <Driver> where is the knife? <Commander> in the sink.", you might output the following top 3 most likely object categories: "answer: Sink, CounterTop, Cabinet". Important: Your output should ONLY a list (3 words seperated by commas) of three object categories from the list above.

What are the top 3 most likely object categories for where to find the target category {INPUT_TARGET_OBJECT} near? Here is the dialogue that may or may not contain relevant information for your answer: {INPUT_DIALOGUE}

answer: 
\end{lstlisting}

\lstset{escapeinside={<@}{@>}, language=Python}
\onecolumn\begin{lstlisting}[caption={Example of a precondition check for the slice macro-action},captionpos=t,label={precond_example}]
if subgoal=="Slice": 
    # contraint check for "slice" macro-action
    if object_tracker.get_label_of_holding()!="Knife":
        # first need to be holding a knife to slice
        program_to_add = [
            'target_knife = InteractionObject("Knife")',
            'target_knife.go_to()',
            'target_knife.pickup()',
        ]
\end{lstlisting}

\lstset{escapeinside={<@}{@>}, language=Python}
\onecolumn\begin{lstlisting}[caption={Example of dialogue input, retrieved examples, and LLM output for a TEACh sample},captionpos=t,label={example1}]
<@\textcolor{orange}{ 
Dialogue input:}@>
<@\textcolor{black}{ 
<Driver> how can I help you today?
<Commander> can you please make me a salad on a clean plate with tomato and cooked potato?
<Driver> does the salad require chopped lettuce?
<Commander> nope!
<Driver> is that all?
<Commander> can you place them on a plate?
<Driver> are they not already on a plate?
}@>


<@\textcolor{red}{Retrieved Examples:}@>
Example 1:
<@\textcolor{black}{ 
dialogue: <Driver> What should I do today? <Commander> hi, make a slice of tomato. <Driver> where is the tomato? <Driver> where is the knife? <Commander> in the sink. <Driver> Tomato sliced. What next? <Commander> slice the potato. <Driver> Where is the potato? <Commander> in the microwave. <Commander> place all salad components on a plate. <Driver> How many slices of potato? <Commander> all salad components need to be place on a plate. <Driver> Where is the plate? <Commander> plate. <Commander> try the tomato piece. <Driver> done. <Commander> we are finished.}@>
Python script:
target_tomato = InteractionObject("Tomato")
target_knife = InteractionObject("Knife") # need knife to slice tomato
target_knife.go_to() # first get knife
target_knife.pickup()
target_tomato.go_to()
target_tomato.slice()
target_tomato_slice1 = InteractionObject("TomatoSliced") # instantiate a tomato slice object after slicing tomato
target_potato = InteractionObject("Potato", landmark = "Microwave") 
target_potato.go_to()
target_potato.slice()
target_potato_slice1 = InteractionObject("PotatoSliced") # instantiate a potato slice object after slicing potato
target_knife.put_down() # put down the knife to free up the agent's hand
target_plate = InteractionObject("Plate") 
target_tomato_slice1.pickup_and_place(target_plate) # pick up the tomato slice and place it on the plate
target_potato_slice1.pickup_and_place(target_plate) # pick up the potato slice and place it on the plate

Example 2:
<@\textcolor{black}{ 
dialogue: <Driver> how can I help? <Commander> please serve 4 slices of tomato on a plate. <Driver> sure. <Driver> where can i find the tomato? <Driver> an knife. <Commander> Tomato on countertop and knife in fridge. <Commander> there should be a plate on the right cupboard by the sink. <Driver> completed. <Commander> great work thanks.}@>
Python script:
target_tomato = InteractionObject("Tomato")
target_knife = InteractionObject("Knife") # need knife to slice tomato
target_knife.go_to() # first get knife
target_knife.pickup()
target_tomato.go_to()
target_tomato.slice()
target_plate = InteractionObject("Plate", landmark = "Sink")
# place 4 slices of the cut tomato on the plate
target_tomato_slice1 = InteractionObject("TomatoSliced") # instantiate first slice of tomato
target_tomato_slice2 = InteractionObject("TomatoSliced") # instantiate second slice of tomato
target_tomato_slice3 = InteractionObject("TomatoSliced") # instantiate third slice of tomato
target_tomato_slice4 = InteractionObject("TomatoSliced") # instantiate fourth slice of tomato
target_tomato_slice1.pickup_and_place(target_plate) # pick up the first tomato slice and place it on the plate
target_tomato_slice2.pickup_and_place(target_plate) # pick up the second tomato slice and place it on the plate
target_tomato_slice3.pickup_and_place(target_plate) # pick up the third tomato slice and place it on the plate
target_tomato_slice4.pickup_and_place(target_plate) # pick up the fourth tomato slice and place it on the plate

Example 3:
<@\textcolor{black}{ 
dialogue: <Driver> hi, what is task. <Commander> make a plate of toast. <Commander> bread in the sink. <Driver> knife. <Commander> on the chair beside the table. <Commander> clean the plate. <Driver> there is a clean one, do i need to clean the other one. <Commander> you can use the clean one. <Driver> done. <Commander> good job. <Driver> :).}@>
Python script:
target_bread = InteractionObject("Bread", landmark = "Sink")
target_knife = InteractionObject("Knife", landmark = "Chair")
target_toaster = InteractionObject("Toaster") # need knife to slice bread
target_knife.go_to() # first get knife
target_knife.pickup()
target_bread.go_to()
target_bread.slice() # slice bread using knife
target_knife.put_down() # put down the knife to free up the agent's hand
target_bread_slice1 = InteractionObject("BreadSliced") # instantiate a bread slice object after slicing bread
target_bread_slice1.pickup_and_place(target_toaster) # pick up the bread slice and place it in the toaster
target_toaster.toggle_on() # turn on toaster to toast bread
target_toaster.toggle_off() # turn off toaster to complete toasting process
# place toast on plate
target_plate = InteractionObject("Plate") 
target_plate.clean()
target_plate.put_down()
target_bread_slice1.pickup_and_place(target_plate) # pick up the toasted bread slice and place it on the plate

<@\textcolor{magenta}{LLM output:}@>
target_tomato = InteractionObject("Tomato")
target_potato = InteractionObject("Potato")
target_plate = InteractionObject("Plate")
target_stove = InteractionObject("StoveBurner")

# Clean the plate
target_plate.go_to()
target_plate.clean()

# Cook the potato
target_potato.go_to()
target_potato.pickup()
target_stove.go_to()
target_potato.place(target_stove)
target_stove.toggle_on()
target_stove.toggle_off()

# Place the cooked potato on the plate
target_potato = InteractionObject("Potato")
target_potato.pickup()
target_plate.go_to()
target_potato.place(target_plate)

# Place the tomato on the plate
target_tomato.go_to()
target_tomato.pickup()
target_plate.go_to()
target_tomato.place(target_plate)
\end{lstlisting}


\onecolumn\begin{lstlisting}[caption={Example of dialogue input, retrieved examples, and LLM output for a TEACh sample},captionpos=t,label={example2}]
<@\textcolor{orange}{ 
Dialogue input:}@>
<@\textcolor{black}{ 
<Driver> what do i do today
<Commander> Hi. Please place two tissue boxes on a table. One is on the gray chair in the corner.
<Commander> The other is under the tv
<Commander> tv*
<Driver> where is the other one
}@>


<@\textcolor{red}{Retrieved Examples:}@>
Example 1:
<@\textcolor{black}{ 
dialogue: <Driver> hi, what is task. <Commander> make a plate of toast. <Commander> bread in the sink. <Driver> knife. <Commander> on the chair beside the table. <Commander> clean the plate. <Driver> there is a clean one, do i need to clean the other one. <Commander> you can use the clean one. <Driver> done. <Commander> good job. <Driver> :).}@>
Python script:
target_bread = InteractionObject("Bread", landmark = "Sink")
target_knife = InteractionObject("Knife", landmark = "Chair")
target_toaster = InteractionObject("Toaster") # need knife to slice bread
target_knife.go_to() # first get knife
target_knife.pickup()
target_bread.go_to()
target_bread.slice() # slice bread using knife
target_knife.put_down() # put down the knife to free up the agent's hand
target_bread_slice1 = InteractionObject("BreadSliced") # instantiate a bread slice object after slicing bread
target_bread_slice1.pickup_and_place(target_toaster) # pick up the bread slice and place it in the toaster
target_toaster.toggle_on() # turn on toaster to toast bread
target_toaster.toggle_off() # turn off toaster to complete toasting process
# place toast on plate
target_plate = InteractionObject("Plate") 
target_plate.clean()
target_plate.put_down()
target_bread_slice1.pickup_and_place(target_plate) # pick up the toasted bread slice and place it on the plate

Example 2:
<@\textcolor{black}{ 
dialogue: <Driver> how can I help? <Commander> please serve 4 slices of tomato on a plate. <Driver> sure. <Driver> where can i find the tomato? <Driver> an knife. <Commander> Tomato on countertop and knife in fridge. <Commander> there should be a plate on the right cupboard by the sink. <Driver> completed. <Commander> great work thanks.}@>
Python script:
target_tomato = InteractionObject("Tomato", landmark = "CounterTop")
target_knife = InteractionObject("Knife", landmark = "Fridge") # need knife to slice tomato
target_knife.go_to() # first get knife
target_knife.pickup()
target_tomato.go_to()
target_tomato.slice()
target_plate = InteractionObject("Plate", landmark = "Sink")
# place 4 slices of the cut tomato on the plate
target_tomato_slice1 = InteractionObject("TomatoSliced") # instantiate first slice of tomato
target_tomato_slice2 = InteractionObject("TomatoSliced") # instantiate second slice of tomato
target_tomato_slice3 = InteractionObject("TomatoSliced") # instantiate third slice of tomato
target_tomato_slice4 = InteractionObject("TomatoSliced") # instantiate fourth slice of tomato
target_tomato_slice1.pickup_and_place(target_plate) # pick up the first tomato slice and place it on the plate
target_tomato_slice2.pickup_and_place(target_plate) # pick up the second tomato slice and place it on the plate
target_tomato_slice3.pickup_and_place(target_plate) # pick up the third tomato slice and place it on the plate
target_tomato_slice4.pickup_and_place(target_plate) # pick up the fourth tomato slice and place it on the plate

Example 3:
<@\textcolor{black}{ 
dialogue: <Driver> How can I help? <Commander> put all the scrub brushes on the counter top. <Driver> where can I find them? <Commander> one is on top of the toilet. <Driver> there is only a cloth. <Driver> I put it on the counter top. <Driver> are there more? <Commander> can you try with the brush to the side of the toilet please? <Driver> okay.}@>
Python script:
target_scrub_brush1 = InteractionObject("ScrubBrush", landmark = "Toilet")
target_counter_top = InteractionObject("CounterTop")
target_scrub_brush1.pickup_and_place(target_counter_top) # pick up the first ScrubBrush and place it on the CounterTop
target_scrub_brush2 = InteractionObject("ScrubBrush", landmark = "Toilet")
target_scrub_brush2.pickup_and_place(target_counter_top) # pick up the second ScrubBrush and place it on the CounterTop

<@\textcolor{magenta}{LLM output:}@>
target_tissue_box1 = InteractionObject("TissueBox", landmark = "Chair")
target_table = InteractionObject("Table")
target_tissue_box1.pickup_and_place(target_table) # pick up the first TissueBox and place it on the Table
target_tissue_box2 = InteractionObject("TissueBox", landmark = "TVStand")
target_tissue_box2.pickup_and_place(target_table) # pick up the second TissueBox and place it on the Table
\end{lstlisting}

\onecolumn\begin{lstlisting}[caption={Example of dialogue input, retrieved examples, and LLM output for a TEACh sample},captionpos=t,label={example3}]
<@\textcolor{orange}{ 
Dialogue input:}@>
<@\textcolor{black}{ 
<Driver> hi how can i help
<Commander> Can you prepare me a coffee in a clean mug
<Commander> There should be a mug on the white table
<Commander> it might need cleaning first
<Commander> that's great
<Driver> are they not already on a plate?}@>


<@\textcolor{red}{Retrieved Examples:}@>
Example 1:
<@\textcolor{black}{ 
dialogue: <Commander> Prepare coffee in a clean mug.}@>
Python script:
target_mug = InteractionObject("Mug")
target_mug.go_to()
target_mug.pickup()
# clean mug in the sink
target_mug.clean()
target_coffee_machine = InteractionObject("CoffeeMachine")
target_coffee_machine.go_to() 
target_mug.place(target_coffee_machine) 
target_coffee_machine.toggle_on() # turn on coffee machine to make coffee
target_coffee_machine.toggle_off() # turn off coffee machine after done

Example 2:
<@\textcolor{black}{ 
dialogue: <Driver> what can i for you today? <Commander> could you boil a potato? <Driver> sure thing! <Driver> are there any pots? <Commander> pots for boiling potato? <Driver> yes. <Commander> just the one that you were holding earlier and a couple others of the same size. <Commander> does it not fit in the sink? <Driver> no. <Commander> see that mug of water next to the pot? <Driver> yes. <Commander> pour the mugs water into the pot. <Driver> thanks. <Commander> you're welcome! <Commander> excellent thank you!}@>
Python script:
target_pot = InteractionObject("Pot")
target_mug = InteractionObject("Mug", landmark = "Pot")
target_mug.go_to()
target_mug.pickup()
target_mug.pour(target_pot)
target_mug.put_down() # put down mug on any location to free up agent's hand
target_potato = InteractionObject("Potato")
target_potato.pickup_and_place(target_pot) # pick up the potato and place it in the pot
target_stove_knob = InteractionObject("StoveKnob") # turn on the stove to boil potato by turning on the stove
target_stove_knob.go_to()
target_stove_knob.toggle_on() # boil water
target_stove_knob.toggle_off() # complete boiling process by turning off

Example 3:
<@\textcolor{black}{ 
dialogue: <Driver> hi, what is task. <Commander> make a plate of toast. <Commander> bread in the sink. <Driver> knife. <Commander> on the chair beside the table. <Commander> clean the plate. <Driver> there is a clean one, do i need to clean the other one. <Commander> you can use the clean one. <Driver> done. <Commander> good job. <Driver> :).}@>
Python script:
target_bread = InteractionObject("Bread", landmark = "Sink")
target_knife = InteractionObject("Knife", landmark = "Chair")
target_toaster = InteractionObject("Toaster", "Toaster") # need knife to slice bread
target_knife.go_to() # first get knife
target_knife.pickup()
target_bread.go_to()
target_bread.slice() # slice bread using knife
target_knife.put_down() # put down the knife to free up the agent's hand
target_bread_slice1 = InteractionObject("BreadSliced") # instantiate a bread slice object after slicing bread
target_bread_slice1.pickup_and_place(target_toaster) # pick up the bread slice and place it in the toaster
target_toaster.toggle_on() # turn on toaster to toast bread
target_toaster.toggle_off() # turn off toaster to complete toasting process
# place toast on plate
target_plate = InteractionObject("Plate") 
target_plate.clean()
target_plate.put_down()
target_bread_slice1.pickup_and_place(target_plate) # pick up the toasted bread slice and place it on the plate


<@\textcolor{magenta}{LLM output:}@>
target_table = InteractionObject("Table")
target_mug = InteractionObject("Mug", landmark = "Table")
target_mug.go_to()
target_mug.pickup()
# clean mug in the sink
target_sink = InteractionObject("Sink")
target_mug.place(target_sink)
target_mug.clean()
target_mug.pickup()
target_coffee_machine = InteractionObject("CoffeeMachine")
target_coffee_machine.go_to() 
target_mug.place(target_coffee_machine) 
target_coffee_machine.toggle_on() # turn on coffee machine to make coffee
target_coffee_machine.toggle_off() # turn off coffee machine after done
\end{lstlisting}
